The Brain Tumor Segmentation (BraTS) Challenge: Local Synthesis of Healthy Brain Tissue via Inpainting

A myriad of algorithms for the automatic analysis of brain MR images is available to support clinicians in their decision-making. For brain tumor patients, the image acquisition time series typically starts with an already pathological scan. This poses problems, as many algorithms are designed to analyze healthy brains and provide no guarantee for images featuring lesions. Examples include, but are not limited to, algorithms for brain anatomy parcellation, tissue segmentation, and brain extraction. To solve this dilemma, we introduce the BraTS inpainting challenge. Here, the participants explore inpainting techniques to synthesize healthy brain scans from lesioned ones. The following manuscript contains the task formulation, dataset, and submission procedure. Later, it will be updated to summarize the findings of the challenge. The challenge is organized as part of the ASNR-BraTS MICCAI challenge.

==> Notes.tex <==
# Important notes/TODO for manuscript goes here 

==> flow/latex_evangelium.tex <==
\section{Latex evangelium}
\label{sec:evangelium}
% \label{sec:formatting}

Look at the .tex file to fully understand this \Cref{sec:evangelium}!


\subsection*{labels and referencing}
\begin{itemize}
    \item label sections that are supposed to be referenced with \label{sec:section_name}
    \item label figures with \label{fig:figure_name}
    \item label tables with \label{tab:table_name}
    \item label equations with \label{eq:equation_name}
    \item reference with \cref{sec:evangelium} or \Cref{sec:evangelium}
\end{itemize}

\subsection*{figures, tables and equations}
\begin{itemize}
    \item use a separate .tex file for each figure/table; this will make the final layout/typesetting process much smoother as we can easily move them around
    \item we put figures in a subfolder for each section called /fig
    \item observe the above label instructions
\end{itemize}

\subsection*{citations}
\begin{itemize}
    \item for citations we use \citep{mckinley2018ensembles} or \citet{mckinley2018ensembles}
\end{itemize}

\subsection*{acronyms}
\begin{itemize}
    \item we define acronyms in /flow/acronyms.tex
    \item for singular acronyms use \eac{CNN} or \eacf{CNN}.
    \item for plural acronyms we use \eacp{CNN} or \eacfp{CNN}.
\end{itemize}

\subsection*{misc but important}
\begin{itemize}
    \item we write in the present tense
    \item we actively use spellcheckers such as Grammarly
    \item we use auto code formatting and lining
    \item we use one line of code for each sentence to enable proper version control with git
\end{itemize}


==> head/author_list_generation/authors.tex <==
\author[1,2,3,73]{Florian  Kofler}
\author[2,4]{Felix  Meissen}
\author[2]{Felix  Steinbauer}
\author[2,4]{Robert  Graf}
\author[5]{Stefan K Ehrlich}
\author[6,7]{Annika  Reinke}
\author[1,8]{Eva  Oswald}
\author[2,9]{Diana  Waldmannstetter}
\author[2,4]{Florian  Hoelzl}
\author[2,10]{Izabela  Horvath}
\author[2,4]{Oezguen  Turgut}
\author[2,4]{Suprosanna  Shit}
\author[1,3]{Christina  Bukas}
\author[9]{Kaiyuan  Yang}
\author[11]{Johannes C. Paetzold}
\author[2,12]{Ezequiel  de da Rosa}
\author[1]{Isra  Mekki}
\author[13,14]{Shankeeth  Vinayahalingam}
\author[15]{Hasan  Kassem}
\author[16]{Juexin  Zhang}
\author[16]{Ke  Chen}
\author[16]{Ying  Weng}
\author[17]{Alicia  Durrer}
\author[17]{Philippe C. Cattin}
\author[17]{Julia  Wolleb}
\author[18]{M. S. Sadique}
\author[18]{M. M. Rahman}
\author[18]{W.  Farzana}
\author[18]{A.  Temtam}
\author[18]{K. M. Iftekharuddin}
\author[19]{Maruf  Adewole}
\author[20,21]{Syed Muhammad Anwar}
\author[22,23,24]{Ujjwal  Baid}
\author[25]{Anastasia  Janas}
\author[22,26]{Anahita Fathi Kazerooni}
\author[27]{Dominic  LaBella}
\author[9,28,29]{Hongwei Bran Li}
\author[30]{Ahmed W Moawad}
\author[31]{Gian-Marco  Conte}
\author[32]{Keyvan  Farahani}
\author[33]{James  Eddy}
\author[34]{Micah  Sheller}
\author[35]{Sarthak  Pati}
\author[15]{Alexandros  Karagyris}
\author[36]{Alejandro  Aristizabal}
\author[33]{Timothy  Bergquist}
\author[33]{Verena  Chung}
\author[22,37]{Russell Takeshi Shinohara}
\author[38]{Farouk  Dako}
\author[39]{Walter  Wiggins}
\author[27]{Zachary  Reitman}
\author[27]{Chunhao  Wang}
\author[20,21]{Xinyang  Liu}
\author[20,21]{Zhifan  Jiang}
\author[40]{Elaine  Johanson}
\author[41]{Zeke  Meier}
\author[26]{Ariana  Familiar}
\author[22,23]{Christos  Davatzikos}
\author[32,42]{John  Freymann}
\author[32,42]{Justin  Kirby}
\author[22,23]{Michel  Bilello}
\author[43]{Hassan M Fathallah-Shaykh}
\author[44,45]{Roland  Wiest}
\author[29]{Jan  Kirschke}
\author[46,47]{Rivka R Colen}
\author[47]{Aikaterini  Kotrotsou}
\author[48]{Pamela  Lamontagne}
\author[49,50]{Daniel  Marcus}
\author[49,50]{Mikhail  Milchenko}
\author[50]{Arash  Nazeri}
\author[51]{Marc-André  Weber}
\author[52]{Abhishek  Mahajan}
\author[22,23]{Suyash  Mohan}
\author[53]{John  Mongan}
\author[53]{Christopher  Hess}
\author[53]{Soonmee  Cha}
\author[53]{Javier  Villanueva-Meyer}
\author[54]{Errol  Colak}
\author[54]{Priscila  Crivellaro}
\author[55]{Andras  Jakab}
\author[56]{Abiodun  Fatade}
\author[57]{Olubukola  Omidiji}
\author[58]{Rachel  Akinola Lagos}
\author[59]{O O Olatunji}
\author[60]{Goldey  Khanna}
\author[27]{John  Kirkpatrick}
\author[61]{Michelle  Alonso-Basanta}
\author[61]{Arif  Rashid}
\author[20]{Miriam  Bornhorst}
\author[22,23,26]{Ali  Nabavizadeh}
\author[62]{Natasha  Lepore}
\author[63]{Joshua  Palmer}
\author[64]{Antonio  Porras}
\author[33]{Jake  Albrecht}
\author[65]{Udunna  Anazodo}
\author[25]{Mariam  Aboian}
\author[39,53]{Evan  Calabrese}
\author[53,66,67]{Jeffrey David Rudie}
\author[20,21]{Marius George Linguraru}
\author[28]{Juan Eugenio Iglesias}
\author[68]{Koen Van Leemput}
\author[23,24,69]{Spyridon  Bakas}
\author[29]{Benedikt  Wiestler}
\author[2,70,71]{Ivan  Ezhov}
\author[1,72]{Marie  Piraud}
\author[9,29,73]{Bjoern H Menze}
\affil[1]{Helmholtz AI, Germany}
\affil[2]{Technical University of Munich, Germany}
\affil[3]{Helmholtz Munich, Germany}
\affil[4]{Klinikum Rechts der Isar, Munich, Germany}
\affil[5]{SETLabs Research GmbH, Healthcare Technologies, Munich, Germany}
\affil[6]{German Cancer Research Center (DKFZ) Heidelberg, Division of Intelligent Medical Systems, Germany}
\affil[7]{German Cancer Research Center (DKFZ) Heidelberg, HI Helmholtz Imaging}
\affil[8]{Institute of Clinical Neuroimmunology, Faculty of Medicine, Ludwig Maximilian University, Munich, Germany}
\affil[9]{University of Zurich, Switzerland}
\affil[10]{Helmholtz Research Center, Munich, Germany}
\affil[11]{Imperial College London, UK}
\affil[12]{Icometrix, Leuven, Belgium}
\affil[13]{Department of Oral and Maxillofacial Surgery, Radboudumc, the Netherlands}
\affil[14]{Department of Artificial Intelligence, Radboud University, the Netherlands}
\affil[15]{MLCommons}
\affil[16]{University of Nottingham Ningbo China, Ningbo 315100, China}
\affil[17]{Center for medical Image Analysis and Navigation, Department of Biomedical Engineering, University of Basel, Allschwil, Switzerland}
\affil[18]{Old Dominion University, Norfolk VA 23529, USA}
\affil[19]{Medical Artificial Intelligence (MAI) Lab, Crestview Radiology, Lagos, Nigeria}
\affil[20]{Children's National Hospital, Washington DC, USA}
\affil[21]{George Washington University, Washington DC, USA}
\affil[22]{Center for AI and Data Science for Integrated Diagnostics (AI2D) \& Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA, USA}
\affil[23]{Department of Radiology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA}
\affil[24]{Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA}
\affil[25]{Yale University, New Haven, CT, USA}
\affil[26]{Children’s Hospital of Philadelphia, University of Pennsylvania, Philadelphia, PA, USA}
\affil[27]{Duke University Medical Center, Department of Radiation Oncology, USA}
\affil[28]{Athinoula A Martinos Center for Biomedical Imaging, Massachusetts General Hospital, Boston, MA, USA}
\affil[29]{Department of Neuroradiology, Technical University of Munich, Munich, Germany}
\affil[30]{Mercy Catholic Medical Center, Darby, PA, USA}
\affil[31]{Department of Radiology, Mayo Clinic, Rochester, MN, USA}
\affil[32]{Cancer Imaging Program, National Cancer Institute, National Institutes of Health, Bethesda, MD 20814, USA}
\affil[33]{Sage Bionetworks, USA}
\affil[34]{Intel/MLCommons}
\affil[35]{IU/MLCommons}
\affil[36]{Factored/MLCommons}
\affil[37]{Center for Clinical Epidemiology and Biostatistics, University of Pennsylvania, Philadelphia, USA}
\affil[38]{Center for Global Health, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA}
\affil[39]{Duke University Medical Center, Department of Radiology, USA}
\affil[40]{PrecisionFDA, U.S. Food and Drug Administration, Silver Spring, MD, USA}
\affil[41]{Booz Allen Hamilton, McLean, VA, USA}
\affil[42]{Leidos Biomedical Research, Inc., Frederick National Laboratory for Cancer Research, Frederick, MD 21701, USA}
\affil[43]{Department of Neurology, The University of Alabama at Birmingham, Birmingham, AL, USA}
\affil[44]{Institute for Surgical Technology and Biomechanics, University of Bern, Bern, Switzerland}
\affil[45]{Support Centre for Advanced Neuroimaging Inselspital, Institute for Diagnostic and Interventional Neuroradiology, Bern University Hospital, Bern, Switzerland}
\affil[46]{University of Pittsburgh Medical Center, PA, USA}
\affil[47]{Department of Diagnostic Radiology, University of Texas MD Anderson Cancer Center, Houston, TX, USA}
\affil[48]{Department of Psychology, Washington University, St. Louis, MO, USA}
\affil[49]{Neuroimaging Informatics and Analysis Center, Washington University, St. Louis, MO, USA}
\affil[50]{Department of Radiology, Washington University, St. Louis, MO, USA}
\affil[51]{Institute of Diagnostic and Interventional Radiology, Pediatric Radiology and Neuroradiology, University Medical Center Rostock, Ernst-Heydemann-Str. 6, 18057 Rostock, Germany}
\affil[52]{Tata Memorial Centre, Homi Bhabha National Institute, Mumbai, India}
\affil[53]{University of California San Francisco, CA, USA}
\affil[54]{University of Toronto, Toronto, ON, Canada}
\affil[55]{University of Debrecen, Hungary}
\affil[56]{Crestview Radiology, Lagos, Nigeria}
\affil[57]{Lagos University Teaching Hospital, Lagos Nigeria}
\affil[58]{University Teaching Hospital, Lagos Nigeria}
\affil[59]{The National Hospital, Abuja, Nigeria}
\affil[60]{Thomas Jefferson University Medical Center, Department of Neurosurgery, Philadelphia, PA, USA}
\affil[61]{Department of Radiation Oncology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA}
\affil[62]{Children’s Hospital of Los Angeles, USA}
\affil[63]{Ohio State University, USA}
\affil[64]{Children’s Hospital Colorado, USA}
\affil[65]{Montreal Neurological Institute (MNI), McGill University, Montreal, QC, Canada}
\affil[66]{University of California San Diego, CA, USA}
\affil[67]{Scripps Clinic, San Diego California}
\affil[68]{Department of Applied Mathematics and Computer Science, Technical University of Denmark, Denmark}
\affil[69]{Analytics (CBICA), University of Pennsylvania, Philadelphia, PA, USA}
\affil[70]{Department of Informatics, Technical University Munich, Germany}
\affil[71]{TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany}
\affil[72]{Helmholtz Munich,  Germany}
\affil[73]{Biomedical Image Analysis \& Machine Learning, Department of Quantitative Biomedicine, University of Zurich, Switzerland}
\setcounter{Maxaffil}{0}
\renewcommand\Authfont{\small}
\renewcommand\Affilfont{\itshape\footnotesize}


==> head/author_list_generation/data_contributor_information_list.tex <==
\author{
% % first block of our own authors
% Florian Kofler \inst{1,2,3,4,\dag}
% Felix Meissen \inst{5,6,\dag}
% Felix Steinbauer \inst{5,\dag}
% Robert Graf \inst{5,6,\dag}
% Eva Oswald \inst{1,48,\dag}
% \\ Ezequiel de la Rosa \inst{5,10,\dag}
% Hongwei Bran Li \inst{20,21,8,\dag}
% Ujjwal Baid \inst{14,15,16,\dag,\ddag}
% Florian A. Hölzl \inst{5,6,\dag}
% Özgün Turgut \inst{5,6,\dag}
% Izabela Horvath \inst{5,7,\dag}
% Diana Waldmannstetter \inst{5,8,\dag}
% Christina Bukas \inst{1,\dag}
% % we expect these people to make a contribution in the future
% Kaiyuan Yang \inst{8,\dag}
% Suprosanna Shit \inst{5,6,\dag}
% Johannes C. Paetzold \inst{9,\dag}
% Israh Mekki \inst{1,\dag}
% Shankeeth Vinayahalingam \inst{49,50,\dag}
% Hasan Kassem \inst{51,\dag}
% Annika Reinke \inst{52,53,\dag}
% % other brats challenge authors
% Maruf Adewole \inst{11,\dag}
% Syed Muhammad Anwar \inst{12,13,\dag}
% Anastasia Janas \inst{17}
% Anahita Fathi Kazerooni \inst{18,14,\dag,\ddag}
% Dominic LaBella \inst{19,\dag}
% Ahmed W Moawad \inst{22}
% Keyvan Farahani \inst{23,\dag,\ddag}
% James Eddy \inst{24,\dag}
% Timothy Bergquist \inst{24,\dag}
% Verena Chung \inst{24,\dag}
% Maria Diaz \inst{24,\dag}
% Byrone Cole \inst{24,\dag}
% Russell Takeshi Shinohara \inst{14,25,\dag}
% Farouk Dako \inst{26,\dag}
% Walter Wiggins \inst{27,\dag,\ddag}
% Zachary Reitman \inst{19,\dag,\ddag}
% Chunhao Wang \inst{19,\dag,\ddag}
% Xinyang Liu \inst{12,13,\dag}
% Zhifan Jiang \inst{12,13,\dag}
% Ariana Familiar \inst{18,\dag}
% Gian-Marco Conte \inst{29,\dag}
% Elaine Johanson \inst{30,\dag}
% Zeke Meier \inst{31,\dag}
% Christos Davatzikos \inst{14,15,\ddag}
% John Freymann \inst{32,23,\ddag}
% Justin Kirby \inst{32,23,\ddag}
% Michel Bilello \inst{14,15,\ddag}
% Hassan M Fathallah-Shaykh \inst{33,\ddag}
% Roland Wiest \inst{34,35,\ddag}
% Jan Kirschke \inst{21,\ddag}
% Rivka R Colen \inst{36,37,\ddag}
% Aikaterini Kotrotsou \inst{37,\ddag}
% Pamela Lamontagne \inst{38,\ddag}
% Daniel Marcus \inst{39,40,\ddag}
% Mikhail Milchenko \inst{39,40,\ddag}
% % data contributors
% Arash Nazeri \inst{40,\ddag}
% Marc-André Weber \inst{41,\ddag}
% Abhishek Mahajan \inst{42,\ddag}
% Suyash Mohan \inst{14,15,\ddag}
% John Mongan \inst{43,\ddag}
% Christopher Hess \inst{43,\ddag}
% Soonmee Cha \inst{43,\ddag}
% Javier Villanueva-Meyer \inst{43,\ddag}
% Errol Colak \inst{44,\ddag}
% Priscila Crivellaro \inst{44,\ddag}
% % seniors
% Andras Jakab \inst{45,\ddag}
% Jake Albrecht \inst{24,\dag}
% Udunna Anazodo \inst{46,\dag}
% Mariam Aboian \inst{17,\dag,\ddag}
% Evan Calabrese \inst{27,43,\dag,\ddag}
% Jeff Rudie \inst{47,43,\dag,\ddag}
% Marius George Linguraru \inst{12,13,\dag,\ddag}
% % our senior authors
% \\ Juan Eugenio Iglesias \inst{20,\dag}
% Koen Van Leemput \inst{28,\dag}
% Spyridon Bakas \inst{14,15,16,\dag,\ddag}
% Daniel Rueckert \inst{5,9,\dag}
% \\ Rolf A. Heckemann \inst{49,\dag}
% Benedikt Wiestler \inst{21,\dag,\ddag}
% Ivan Ezhov \inst{2, \dag}
% Marie Piraud \inst{1,\dag}
% Bjoern Menze \inst{8,\dag,\ddag}
% }
Florian Kofler \inst{1,4,11\dag}
Felix Meissen \inst{5,6,\dag}
Felix Steinbauer \inst{5,\dag}
Robert Graf \inst{5,6,\dag}
Eva Oswald \inst{1,64,\dag}
Diana Waldmannstetter \inst{5,8,\dag}
Florian Hoelzl \inst{5,6,\dag}
Izabela Horvath \inst{5,7,\dag}
Oezguen Turgut \inst{5,6,\dag}
Suprosanna Shit \inst{5,6,\dag}
Christina Bukas \inst{1,11\dag}
Kaiyuan Yang \inst{8,\dag}
Johannes C. Paetzold \inst{9,\dag}
Ezequiel de da Rosa \inst{5,10,\dag}
Isra Mekki \inst{1,\dag}
Shankeeth  Vinayahalingam \inst{12,13,\dag}
Hasan Kassem \inst{14,\dag}
Annika Reinke \inst{15,16,\dag}
Maruf Adewole \inst{17,\dag}
Syed Muhammad Anwar \inst{18,19,\dag}
Ujjwal Baid \inst{20,21,22,\dag,\ddag}
Anastasia Janas \inst{23}
Anahita Fathi Kazerooni \inst{24,20,\dag,\ddag}
Dominic LaBella \inst{25,\dag}
Hongwei Bran Li \inst{26,27,8,\dag}
Ahmed W Moawad \inst{28}
Gian-Marco Conte \inst{29,\dag}
Juan Eugenio Iglesias \inst{26,\dag}
Keyvan Farahani \inst{30,\dag,\ddag}
James Eddy \inst{31,\dag}
Timothy Bergquist \inst{31,\dag}
Verena Chung \inst{31,\dag}
Russell Takeshi Shinohara \inst{20,32,\dag}
Farouk Dako \inst{33,\dag}
Walter Wiggins \inst{34,\dag,\ddag}
Zachary Reitman \inst{25,\dag,\ddag}
Chunhao Wang \inst{25,\dag,\ddag}
Xinyang Liu \inst{18,19,\dag}
Zhifan Jiang \inst{18,19,\dag}
Elaine Johanson \inst{36,\dag}
Zeke Meier \inst{37,\dag}
Ariana Familiar \inst{24,\dag}
Christos Davatzikos \inst{20,21,\ddag}
John Freymann \inst{38,30,\ddag}
Justin Kirby \inst{38,30,\ddag}
Michel Bilello \inst{20,21,\ddag}
Hassan M Fathallah-Shaykh \inst{39,\ddag}
Roland Wiest \inst{40,41,\ddag}
Jan Kirschke \inst{27,\ddag}
Rivka R Colen \inst{42,43,\ddag}
Aikaterini Kotrotsou \inst{43,\ddag}
Pamela Lamontagne \inst{44,\ddag}
Daniel Marcus \inst{45,46,\ddag}
Mikhail Milchenko \inst{45,46,\ddag}
Arash Nazeri \inst{46,\ddag}
Marc-André Weber \inst{47,\ddag}
Abhishek Mahajan \inst{48,\ddag}
Suyash Mohan \inst{20,21,\ddag}
John Mongan \inst{49,\ddag}
Christopher Hess \inst{49,\ddag}
Soonmee Cha \inst{49,\ddag}
Javier Villanueva-Meyer \inst{49,\ddag}
Errol Colak \inst{50,\ddag}
Priscila Crivellaro \inst{50,\ddag}
Andras Jakab \inst{51,\ddag}
Abiodun Fatade \inst{52,\ddag}
Olubukola Omidiji \inst{53,\ddag}
Rachel Akinola \inst{53,\ddag}
O O Olatunji \inst{54,\ddag}
Goldey Khanna \inst{55,\ddag}
John Kirkpatrick \inst{25,\ddag}
Michelle Alonso-Basanta \inst{56,\ddag}
Arif Rashid \inst{56,\ddag}
Miriam Bornhorst \inst{18,\ddag}
Ali Nabavizadeh \inst{24,20,21,\ddag}
Natasha Lepore \inst{57,\ddag}
Joshua Palmer \inst{58,\ddag}
Antonio Porras \inst{59,\ddag}
Jake Albrecht \inst{31,\dag}
Udunna Anazodo \inst{60,\dag}
Mariam Aboian \inst{23,\dag,\ddag}
Evan Calabrese \inst{34,49,\dag,\ddag}
Jeffrey David Rudie \inst{62,49,63,\dag,\ddag}
Marius George Linguraru \inst{18,19,\dag,\ddag}
Koen Van Leemput \inst{35,\dag}
Spyridon Bakas \inst{20,21,22,\dag,\ddag}
Benedikt Wiestler \inst{27,\dag,\ddag}
Ivan Ezhov \inst{2,3,5,\dag}
Marie Piraud \inst{1,11\dag}
Bjoern H Menze \inst{8,27,61,\dag,\ddag}
}
\authorrunning{Kofler \textit{et al.}}



\institute{\scriptsize{
% affiliations
% Helmholtz AI, Helmholtz Munich, Germany \and  % 1
% Department of Informatics, Technical University Munich, Germany \and  % 2
% TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany \and  % 3
% Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany \and  % 4
% Technical University of Munich, Germany \and  % 5
% Klinikum Rechts der Isar, Munich, Germany \and  % 6
% Helmholtz Research Center, Munich, Germany \and  % 7
% University of Zurich, Switzerland \and  % 8
% Imperial College, London, UK \and  % 9
% Icometrix, Leuven, Belgium \and  % 10
% Medical Artificial Intelligence (MAI) Lab, Crestview Radiology, Lagos, Nigeria \and  % 11
% Children's National Hospital, Washington DC, USA \and  % 12
% George Washington University, Washington DC, USA \and  % 13
% Center for AI and Data Science for Integrated Diagnostics (AI2D) I\& Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA, USA \and  % 14
% Department of Radiology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA \and  % 15
% Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA \and  % 16
% Yale University, New Haven, CT, USA \and  % 17
% Children’s Hospital of Philadelphia, University of Pennsylvania, Philadelphia, PA, USA \and  % 18
% Duke University Medical Center, Department of Radiation Oncology, USA \and  % 19
% Athinoula A Martinos Center for Biomedical Imaging, Massachusetts General Hospital, Boston, MA, USA \and  % 20
% Department of Neuroradiology, Technical University of Munich, Munich, Germany \and  % 21
% Mercy Catholic Medical Center, Darby, PA, USA \and  % 22
% Cancer Imaging Program, National Cancer Institute, National Institutes of Health, Bethesda, MD 20814, USA \and  % 23
% Sage Bionetworks, USA \and  % 24
% Center for Clinical Epidemiology and Biostatistics, University of Pennsylvania, Philadelphia, USA \and  % 25
% Center for Global Health, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA \and  % 26
% Duke University Medical Center, Department of Radiology, USA \and  % 27
% Department of Applied Mathematics and Computer Science, Technical University of Denmark, Denmark \and  % 28
% Mayo Clinic, MN, USA \and  % 29
% PrecisionFDA, U.S. Food and Drug Administration, Silver Spring, MD, USA \and  % 30
% Booz Allen Hamilton, McLean, VA, USA \and  % 31
% Leidos Biomedical Research, Inc., Frederick National Laboratory for Cancer Research, Frederick, MD 21701, USA \and  % 32
% Department of Neurology, The University of Alabama at Birmingham, Birmingham, AL, USA \and  % 33
% Institute for Surgical Technology and Biomechanics, University of Bern, Bern, Switzerland \and  % 34
% Support Centre for Advanced Neuroimaging Inselspital, Institute for Diagnostic and Interventional Neuroradiology, Bern University Hospital, Bern, Switzerland \and  % 35
% University of Pittsburgh Medical Center, PA, USA \and  % 36
% Department of Diagnostic Radiology, University of Texas MD Anderson Cancer Center, Houston, TX, USA \and  % 37
% Department of Psychology, Washington University, St. Louis, MO, USA \and  % 38
% Neuroimaging Informatics and Analysis Center, Washington University, St. Louis, MO, USA \and  % 39
% Department of Radiology, Washington University, St. Louis, MO, USA \and  % 40
% Institute of Diagnostic and Interventional Radiology, Pediatric Radiology and Neuroradiology, University Medical Center Rostock, Ernst-Heydemann-Str. 6, 18057 Rostock, Germany \and  % 41
% Tata Memorial Centre, Homi Bhabha National Institute, Mumbai, India \and  % 42
% University of California San Francisco, CA, USA \and  % 43
% University of Toronto, Toronto, ON, Canada \and  % 44
% University of Debrecen, Hungary \and  % 45
% Montreal Neurological Institute (MNI), McGill University, Montreal, QC, Canada \and  % 46
% UCSD, USA \and % 47
% Institute of Clinical Neuroimmunology, Faculty of Medicine, Ludwig Maximilian University, Munich, Germany \and %48
% Department of Medical Radiation Sciences, University of Gothenburg, Sweden \and %49
% Department of Oral and Maxillofacial Surgery, Radboudumc, the Netherlands  \and  % 50
% Department of Artificial Intelligence, Radboud University, the Netherlands  \and  % 51
% MLCommons \and  % 52
% German Cancer Research Center (DKFZ) Heidelberg, Division of Intelligent Medical Systems, Germany \and  % 53
% German Cancer Research Center (DKFZ) Heidelberg, HI Helmholtz Imaging \and  % 54
% end block
Helmholtz AI, Germany \and  % 1
Department of Informatics, Technical University Munich, Germany \and  % 2
TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany \and  % 3
Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany \and  % 4
Technical University of Munich, Germany \and  % 5
Klinikum Rechts der Isar, Munich, Germany \and  % 6
Helmholtz Research Center, Munich, Germany \and  % 7
University of Zurich, Switzerland \and  % 8
Imperial College, London, UK \and  % 9
Icometrix, Leuven, Belgium \and  % 10
Helmholtz Munich,  Germany \and  % 11
Department of Oral and Maxillofacial Surgery, Radboudumc, the Netherlands  \and  % 12
Department of Artificial Intelligence, Radboud University, the Netherlands  \and  % 13
MLCommons \and  % 14
German Cancer Research Center (DKFZ) Heidelberg, Division of Intelligent Medical Systems, Germany \and  % 15
German Cancer Research Center (DKFZ) Heidelberg, HI Helmholtz Imaging \and  % 16
Medical Artificial Intelligence (MAI) Lab, Crestview Radiology, Lagos, Nigeria \and  % 17
Children's National Hospital, Washington DC, USA \and  % 18
George Washington University, Washington DC, USA \and  % 19
Center for AI and Data Science for Integrated Diagnostics (AI2D) \& Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA, USA \and  % 20
Department of Radiology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA \and  % 21
Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA \and  % 22
Yale University, New Haven, CT, USA \and  % 23
Children’s Hospital of Philadelphia, University of Pennsylvania, Philadelphia, PA, USA \and  % 24
Duke University Medical Center, Department of Radiation Oncology, USA \and  % 25
Athinoula A Martinos Center for Biomedical Imaging, Massachusetts General Hospital, Boston, MA, USA \and  % 26
Department of Neuroradiology, Technical University of Munich, Munich, Germany \and  % 27
Mercy Catholic Medical Center, Darby, PA, USA \and  % 28
Department of Radiology, Mayo Clinic, Rochester, MN, USA \and  % 29
Cancer Imaging Program, National Cancer Institute, National Institutes of Health, Bethesda, MD 20814, USA \and  % 30
Sage Bionetworks, USA \and  % 31
Center for Clinical Epidemiology and Biostatistics, University of Pennsylvania, Philadelphia, USA \and  % 32
Center for Global Health, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA \and  % 33
Duke University Medical Center, Department of Radiology, USA \and  % 34
Department of Applied Mathematics and Computer Science, Technical University of Denmark, Denmark \and  % 35
PrecisionFDA, U.S. Food and Drug Administration, Silver Spring, MD, USA \and  % 36
Booz Allen Hamilton, McLean, VA, USA \and  % 37
Leidos Biomedical Research, Inc., Frederick National Laboratory for Cancer Research, Frederick, MD 21701, USA \and  % 38
Department of Neurology, The University of Alabama at Birmingham, Birmingham, AL, USA \and  % 39
Institute for Surgical Technology and Biomechanics, University of Bern, Bern, Switzerland \and  % 40
Support Centre for Advanced Neuroimaging Inselspital, Institute for Diagnostic and Interventional Neuroradiology, Bern University Hospital, Bern, Switzerland \and  % 41
University of Pittsburgh Medical Center, PA, USA \and  % 42
Department of Diagnostic Radiology, University of Texas MD Anderson Cancer Center, Houston, TX, USA \and  % 43
Department of Psychology, Washington University, St. Louis, MO, USA \and  % 44
Neuroimaging Informatics and Analysis Center, Washington University, St. Louis, MO, USA \and  % 45
Department of Radiology, Washington University, St. Louis, MO, USA \and  % 46
Institute of Diagnostic and Interventional Radiology, Pediatric Radiology and Neuroradiology, University Medical Center Rostock, Ernst-Heydemann-Str. 6, 18057 Rostock, Germany \and  % 47
Tata Memorial Centre, Homi Bhabha National Institute, Mumbai, India \and  % 48
University of California San Francisco, CA, USA \and  % 49
University of Toronto, Toronto, ON, Canada \and  % 50
University of Debrecen, Hungary \and  % 51
Crestview Radiology, Lagos, Nigeria \and  % 52
Lagos University Teaching Hospital, Lagos Nigeria. \and  % 53
The National Hospital, Abuja, Nigeria \and  % 54
Thomas Jefferson University Medical Center, Department of Neurosurgery, Philadelphia, PA, USA \and  % 55
Department of Radiation Oncology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, PA, USA \and  % 56
Children’s Hospital of Los Angeles, USA \and  % 57
Ohio State University, USA \and  % 58
Children’s Hospital Colorado, USA \and  % 59
Montreal Neurological Institute (MNI), McGill University, Montreal, QC, Canada \and  % 60
Biomedical Image Analysis \& Machine Learning, Department of Quantitative Biomedicine, University of Zurich, Switzerland \and  % 61
University of California San Diego, CA, USA \and  % 62
Scripps Clinic, San Diego California \and  % 63
Institute of Clinical Neuroimmunology, Faculty of Medicine, Ludwig Maximilian University, Munich, Germany \and  % 64
\\
\textsuperscript{\dag} People involved in the organization of the challenge.\\
\textsuperscript{\ddag} People contributing data from their institutions.\\
} 
Corresponding author: \email{\{florian.kofler@tum.de\}}}

==> head/plain_author_list_for_arxiv_v1.tex <==
Florian Kofler, Felix Meissen, Felix Steinbauer, Robert Graf, Eva Oswald, Ezequiel de da Rosa, Hongwei Bran Li, Ujjwal Baid, Florian Hoelzl, Oezguen Turgut, Izabela Horvath, Diana Waldmannstetter, Christina Bukas, Maruf Adewole, Syed Muhammad Anwar, Anastasia Janas, Anahita Fathi Kazerooni, Dominic LaBella, Ahmed W Moawad, Keyvan Farahani, James Eddy, Timothy Bergquist, Verena Chung, Russell Takeshi Shinohara, Farouk Dako, Walter Wiggins,Zachary Reitman, Chunhao Wang, Xinyang Liu, Zhifan Jiang, Ariana Familiar, Gian-Marco Conte, Elaine Johanson, Zeke Meier, Christos Davatzikos, John Freymann, Justin Kirby, Michel Bilello, Hassan M Fathallah-Shaykh, Roland Wiest, Jan Kirschke, Rivka R Colen, Aikaterini Kotrotsou, Pamela Lamontagne, Daniel Marcus, Mikhail Milchenko, Arash Nazeri, Marc-André Weber, Abhishek Mahajan, Suyash Mohan, John Mongan, Christopher Hess, Soonmee Cha, Javier Villanueva-Meyer, Errol Colak, Priscila Crivellaro, Andras Jakab, Jake Albrecht, Udunna Anazodo, Mariam Aboian, Juan Eugenio Iglesias, Koen Van Leemput, Spyridon Bakas, Daniel Rueckert, Benedikt Wiestler, Ivan Ezhov, Marie Piraud, Bjoern Menze

==> overleaf_emails.tex <==
ivan.ezhov@tum.de
florian.sebastian.kofler@gmail.com

j.paetzold@ic.ac.uk

felix.steinbauer@web.de
felix.meissen@tum.de
o.eva@t-online.de

robert.graf@tum.de

christina.bukas@helmholtz-muenchen.de

% 2do:
b.wiestler@tum.de
